Novel Hybrid-Learning Algorithms for Improved Millimeter-Wave Imaging Systems

Increasing attention is being paid to millimeter-wave (mmWave), 30 GHz to 300 GHz, and terahertz (THz), 300 GHz to 10 THz, sensing applications including security sensing, industrial packaging, medical imaging, and non-destructive testing. Traditional methods for perception and imaging are challenged by novel data-driven algorithms that offer improved resolution, localization, and detection rates. Over the past decade, deep learning technology has garnered substantial popularity, particularly in perception and computer vision applications. Whereas conventional signal processing techniques are more easily generalized to various applications, hybrid approaches where signal processing and learning-based algorithms are interleaved pose a promising compromise between performance and generalizability. Furthermore, such hybrid algorithms improve model training by leveraging the known characteristics of radio frequency (RF) waveforms, thus yielding more efficiently trained deep learning algorithms and offering higher performance than conventional methods. This dissertation introduces novel hybrid-learning algorithms for improved mmWave imaging systems applicable to a host of problems in perception and sensing. Various problem spaces are explored, including static and dynamic gesture classification; precise hand localization for human computer interaction; high-resolution near-field mmWave imaging using forward synthetic aperture radar (SAR); SAR under irregular scanning geometries; mmWave image super-resolution using deep neural network (DNN) and Vision Transformer (ViT) architectures; and data-level multiband radar fusion using a novel hybrid-learning architecture. Furthermore, we introduce several novel approaches for deep learning model training and dataset synthesis.

==> my_papers.tex <==
J. W. Smith, M. E. Yanik and M. Torlak, ``Near-field MIMO-ISAR millimeter-wave imaging,'' \textit{Proc. IEEE Radar Conf.}, Florence, Italy, Sep. 2020, pp. 1-6..

J. W. Smith, S. Thiagarajan, R. Willis, Y. Makris, and M. Torlak, ``Improved static hand gesture classification on deep convolutional neural networks using novel sterile training technique,'' \textit{IEEE Access}, vol. 9, pp. 10893–10902, Jan. 2021.

J. W. Smith, O. Furxhi, M. Torlak, ``An {FCNN}-based super-resolution {mmWave} radar framework for contactless musical instrument interface,'' in \textit{IEEE Trans. on Multimedia}, May 2021.

J. W. Smith and M. Torlak, ``Efficient \mbox{3-D} near-field MIMO-SAR imaging for irregular scanning geometries,'' \textit{IEEE Access}, vol. 10, pp 10283-10294, Jan. 2022.


J. W. Smith, Y. Alimam, G. Vedula, and M. Torlak, ``A vision transformer approach for efficient near-field SAR super-resolution under array perturbation,'' in \textit{Proc. IEEE TSWMCS}, submitted for publication.

C. Vasieleiou, J. W. Smith, S. Thiagarajan, M. Nigh, Y. Makris, and M. Torlak, ``Efficient DNN-based super resolution algorithms for mmWave mobile radar imaging,'' in \textit{Proc. IEEE ICIP}, submitted for publication.

J. W. Smith and M. Torlak, ``Deep learning-based multiband signal fusion for 3-D SAR super-resolution,'' \textit{IEEE Trans. Image Process.}, submitted for publication.

J. W. Smith and M. Torlak, ``Survey of emerging systems and algorithms for near-field THz SAR imaging,'' \textit{IEEE Trans. THz Sci. Technol.}, to be submitted.
